Data balancing for boosting performance of low-frequency classes in Spoken Language Understanding

Despite the fact that data imbalance is becoming more and more common in real-world Spoken Language Understanding (SLU) applications, it has not been studied extensively in the literature. To the best of our knowledge, this paper presents the first systematic study on handling data imbalance for SLU. In particular, we discuss the application of existing data balancing techniques for SLU and propose a multi-task SLU model for intent classification and slot filling. Aiming to avoid over-fitting, in our model methods for data balancing are leveraged indirectly via an auxiliary task which makes use of a class-balanced batch generator and (possibly) synthetic data. Our results on a real-world dataset indicate that i) our proposed model can boost performance on low frequency intents significantly while avoiding a potential performance decrease on the head intents, ii) synthetic data are beneficial for bootstrapping new intents when realistic data are not available, but iii) once a certain amount of realistic data becomes available, using synthetic data in the auxiliary task only yields better performance than adding them to the primary task training data, and iv) in a joint training scenario, balancing the intent distribution individually improves not only intent classification but also slot filling performance.

==> sections/exp.tex <==
% !TEX root = ../coling2020.tex     
\section{Experiments}
%In this section, we first describe the utilized Alexa SLU datasets and subsequently the experimental settings.
In this section, we describe our experiments comparing different data balancing techniques on a real-world German SLU dataset. 
\subsection{Datasets}
An overview of the dataset statistics is provided in Table \ref{tbl:data}.

\begin{table}%[ht]
\centering%\small
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Dataset} & \textbf{Snooze} & \textbf{Browse} & \textbf{Cancel} & \textbf{Head I.}\\
\hline
\hline
Train & 40 & 16& --& 166,493\\
Val. & 10 & 4 & -- & 20,846\\
Test & 449 & 634 & 623& 20,710 \\
NMT data & 20,285 & 7,855& 2,657 & --\\
\hline
\end{tabular}
\caption{Number of samples for three simulated low-frequency intents and the remaining seven intents (head intents).}
% SnoozeNotificationIntent, BrowseReminderIntent. and CancelReminderIntent. have 50, 20 and 0 samples in training and validation datasets, respectively.}
\label{tbl:data}
%\vspace{-0.3cm}
\vspace{-0.9cm}
\end{table}

\subsubsection{SLU realistic data} We extracted a random data sample
from a commercial German SLU system; the data are representative of requests to voice-controlled devices and were manually annotated with intent and slot labels. The sample is from the \emph{Notifications} domain and comprises 351.066 samples. We split the dataset into 80\% train, 10\% validation and 10\% test data. The data are highly imbalanced for intent classes with a long-tail distribution, where the smallest classes comprise a single sample only. Due to the small amount of test instances for low-frequency intents, we cannot reliably evaluate performance for them. Therefore, we created an artificial set up to study intent bootstrapping in a systematic way. In particular, we first removed data of all intents having fewer than 1,000 samples, leaving 10 classes. This ensures that at least 100 test samples are available per intent, which are needed to measure performance reliably in a large-scale set up. We selected the three intents with the lowest frequency from the remaining intents to simulate intent bootstrapping and filtered out all of their samples from the train and validation datasets. To simulate the growing data amounts per class in a developing system, where new features are added over time, we randomly sampled a different amount for each of the three intents and re-added 80\% and 20\% to the filtered train and validation datasets, respectively. We added 0, 20 and 50 samples for \emph{CancelReminderIntent}, \emph{BrowseReminderIntent} and \emph{SnoozeNotificationIntent}, respectively. 
This is the \textit{main} data set for our SLU experiments.
\subsubsection{Machine-translated data} We translated data from an English NLU system into German using a transformer-based neural machine translation (NMT) system trained with Sockeye \cite{Sockeye:17}. The NMT system was trained on 4,000 segments of internal data as well as 28,733,606 segments of publicly available data; slot labels were projected from the English source utterances to the German translations using the alignment model \emph{fast\_align} \cite{fastalign}. The number of NMT-generated samples is 2,657, 7,855 and 20,285 for \emph{CancelReminderIntent}, \emph{BrowseReminderIntent} and \emph{SnoozeNotificationIntent}, respectively. This data set is used for \textit{data augmentation} of low-frequency classes in our experiments.


%\textbf{Publicly available SLU data.}
%The ATIS dataset \cite{conf/slt/TurHH10} is a small-scale dataset, which has been widely used in SLU research. It consists of audio recordings and corresponding annotated transcriptions in English of people making flight reservations. We use the version provided by \newcite{N18-2118}, in which the training, validation and test sets contain 4.478, 500 and 893  utterances, respectively. The data are imbalanced, with the smallest intent classes comprising a single sample only. %The word vocabulary of the dataset is of size 778.

\subsection{Models}
We train and evaluate the following models on our SLU data:
\begin{itemize}
    \setlength{\parskip}{-3pt}
    \item \emph{Baseline}: The standard model without any data imbalance handling technique; this baseline is obtained by training the primary task individually on SLU training data.
    \item \emph{Over-sampling}: Common random over-sampling method; for each intent class, SLU training data are up-sampled to the number of samples in the head class. The model is then obtained by training the primary task individually on the up-sampled training set.
    \item \emph{Balanced-loss}: Common re-weighting method with DNN loss; The cross entropy loss of IC is balanced by using class frequencies. The model is obtained by training the primary task individually on SLU training data.
    \item \emph{CBG}: The primary task is trained individually on SLU training data using the class-balanced batch generator.
    \item \emph{Mul.-CBG}: Proposed method \textit{without} data augmentation; an auxiliary task with class-balanced batch generator (without using machine translated data) is applied.
    \item \emph{Data-aug.}: Common training data augmentation method; SLU training data are augmented with all of the available synthetic NMT data for low-frequency classes. The primary task model is then trained individually on the augmented SLU training set.
    \item \emph{Data-aug.+Over-sampl.}: Combination of the above \emph{data-aug.} and \emph{over-sampling} approaches. SLU training data are first augmented by adding all of the available synthetic NMT data for low-frequency classes and subsequently up-sampled as in \emph{over-sampling}. The model is then obtained by training the primary task individually on the up-sampled and augmented training set.
    \item \emph{Data-aug.+Balanced-loss}: Combination of the above \emph{data-augmentation} and \emph{balanced-loss} approaches. SLU training data is augmented by adding all of the available synthetic NMT data for low-frequency classes. The model is then obtained by training the primary task individually on augmented training data with balanced loss.
    \item \emph{Data-aug.+CBG}: Combination of the above \emph{data-augmentation} and \emph{CBG} approaches. SLU training data is augmented by adding all of the available synthetic NMT data. The primary task model is then trained individually on the augmented SLU training set using a class-balanced batch generator.
    \item \emph{Mul.-CBG+Data-aug.}: Proposed method \textit{with} data augmentation; the auxiliary task with class-balanced batch generator is applied on the NMT-augmented dataset.
\end{itemize}
%While \emph{Ours} and  \emph{Ours+Data-aug.} are trained using both of primary and auxiliary tasks, the other models are trained with only the primary task in our model.
\subsection{Settings}
In our experiments, we use pre-trained multilingual BERT \cite{mbert} (size 768), and max-pooling for sentence representation. Each of our decoders has 2 dense layers of size 768 with gelu activation. The dropout values used in IC and SF decoders are 0.5 and 0.2, respectively. For optimization, we use Adam optimizer with learning rate 0.1 and a Noam learning rate scheduler. We trained our model 
%for 10 epochs 
with batch size of 64.

Following Gaspers et al. (2018) \cite{gaspers2018}, we use a semantic error rate, which measures IC and SF jointly and is defined as follows:
\begin{equation}
\textrm{\emph{SemER}} = \frac{\#(\textrm{slot+intent errors})}{\#\textrm{slots in reference + 1}}\end{equation}


%\subsection{Results}
%In the following, we first conduct a systematic study regarding data balancing for large-scale SLU on our Alexa feature bootstrapping set up. Subsequently, we explore on the ATIS benchmark datset whether using an auxiliary task with class-balanced batch geSFator can improve upon a SOTA SLU model.
%\subsection{Feature bootstrapping on internal data}
%We compare our method to common data balancing methods, and we study application with NMT data augmentation for low-frequency classes:
%\begin{itemize}
%    \setlength{\parskip}{-3pt}
%    \item \emph{RSS}: Conventional supervised baseline with regular  randomly  sampled  batches as inputs. This is %the standard model without any data imbalance handling technique.
%    \item \emph{ROS}: Common random over-sampling method; for each intent class, data are up-sampled to the number of samples in the head class.
%    \item \emph{NMT}: Common training data augmentation method; training data are augmented with NMT data for low-frequency classes.
%    \item \emph{WL}: Common re-weighting method with DNN loss; 
%    \item \emph{RSS-CBG}: Proposed method; an auxiliary task with class-balanced batch geSFator is applied. SLU data is used in both tasks.
%    \item \emph{RSS-CBG\_NMT}: Same as above, but the auxiliary task with class-balanced batch geSFator is applied on \emph{NMT}.
%\end{itemize}
    
%Results for the different methods on our feature bootstrapping set up are shown in Table \ref{tbl:fb_results}.

%\begin{table}[ht]
%\centering%\small
%\begin{tabular}{l|l|l|l|l}
%\hline
%\textbf{Method} & \textbf{SnoozeN.} & \textbf{BrowseR.} & \textbf{CancelR.} & \textbf{Head intents}\\
%\hline
%\hline
%baseline: \emph{RSS} & 22.56 & 64.43 & 55.58 & 4.55\\
%\hline
%\emph{ROS} + \emph{RSS} &15.65 & 28.33 & 46.26 & 4.87\\
%\emph{WL} + \emph{RSS}& 15.24 & 38.42 & 46.26 & 5.07\\
% CBG 6
%\emph{RSS-CBG}  &21.75 & 34.94 & 50.06 & 4.5\\
%\hline
%\emph{NMT} + \emph{RSS} + \emph{RSS} & 76.02 & 43.39 & 31.22 & 4.54\\
%\emph{NMT} + \emph{ROS} + \emph{RSS} & 15.04 & 40.49 & 30.58 & 4.69 \\
%\emph{NMT} + \emph{WL} + \emph{RSS}& 9.55 & 43.18 & 28.11 &   4.73\\
% CBG 5
%\hline
%\emph{RSS-CBG\_NMT} & 15.85 & 42.39 & 54.12 & 4.53\\
%\emph{base},  & mBERT on \emph{base} +  & \multirow{2}{*}{15.85} & \multirow{2}{*}{42.39} & \multirow{2}{*}{54.12} & \multirow{2}{*}{4.53}\\
%\emph{base+MT} & CBG on \emph{base+MT} &&&& \\
%\hline
%\end{tabular}
%\caption{SemER on three low-frequency intents and on the head intents for data balancing methods on internal data.}
% SnoozeNotificationIntent, BrowseReminderIntent. and CancelReminderIntent. have 50, 20 and 0 samples in training and validation datasets, respectively.}
%\label{tbl:fb_results}
%\vspace{-0.3cm}
%\end{table}

%As can be seen, performance for all of the low-frequency intents can be improved just by balancing the regular training data. However, for both random over-sampling and weighted losses the boost in performance comes at the cost of a relative increase of 7\% and 11\%, respectively, in \emph{SemER} for the head intents. As head intents are much more frequently used by customers, and the customers are used to their comparatively high performance already, such a decrease in performance is typically not acceptable. By contrast, \emph{RSS-CBG} boosts performance for all low-frequency features, yielding up to 46\% relative reduction in \emph{SemER}, without overfitting on the low-frequency classes.
%. In particular, for the head classes CBG yields a slightly lower SemER of 4.5\% compared to 4.55\% achieved by the baseline system. 
%Interestingly, the intent-based data balancing methods also improve SF performance, as indicated by the results for \emph{CancelReminderIntent}. Recall that there are no samples for this intent in the regular training data. Hence, the intent cannot be recognized by the model, yielding an intent classification accuracy of 0.0; in fact, the improvements in \emph{SemER} for \emph{CancelReminderIntent} are solely resulting from improved SF performance. We attribute this improvement to the fact that slots are shared across several intents and may benefit from intent-based data balancing, as we are using a multi-task model for IC and SF.  
%his intent represents a completely new feature, where no training data is available yet, and hence -- as long as NMT intent data are not added -- the intent cannot be recognized by the model, yielding an intent classification accuracy of 0.0; in fact, the improvements in SemER for \emph{CancelReminderIntent} are solely resulting from improved slot filling performance. We attribute this improvement to the fact that slots are shared across several intents and may benefit from intent-based data balancing, as we are using a multi-task model for intent classification and slot filling.  
 
%As expected, performance is improved when adding NMT data to \emph{CancelReminderIntent}, which didn't have any intent samples beforehand. However, for \emph{SnoozeNotificationIntent}, which already had 50 intent samples, adding NMT data yields a large increase in \emph{SemER} from 22.5\% to 76.02\%. This highlights the fact that in an evolving system one needs to be careful with maintaining synthetic data. They can be very useful to bootstrap new features when no or few customer feature data are available. However, as they are typically of comparatively low quality, they can decrease performance when they are kept while more and more customer feature data become available. While random over-sampling and weighted losses can mitigate this problem and improve performance on low-frequency classes, this again comes at the cost of a decrease in performance for the head intents.

%\emph{RSS-CBGN\_MT} indicates performance when NMT data are not added to the primary task training data, but used in the auxiliary task during training only. For \emph{SnoozeNotificationIntent} and \emph{BrowseReminderIntent}, which already have a small number of samples in the regular training data, performance is improved compared to adding NMT data to the primary task training data without overfitting on the head classes. For \emph{SnoozeNotificationIntent} performance for \emph{RSS-CBSmodel.exported_block_listN\_MT} is better than both \emph{RSS-CBS} on the regular data and \emph{NMT} + \emph{RSS}. This suggests that once a certain amount of regular intent data becomes available, it's beneficial to leverage NMT data only with \emph{RSS-CBSN\_MT}. However, for intents without regular training data standard NMT data augmentation is preferable, as the intent cannot be recognized otherwise. Note that this is the case for \emph{CancelReminderIntent} in this experiment. 

%Overall conclusion is that across all features with CBS we can improve low-freq features while not decreasing (actually increasing) overall performance, and also some MT insights, e.g. that when some live data are available balancing with MT can be more useful than adding MT (which can decrease performance)

%\subsection{Comparison to the state-of-the-art}
%We evaluated our approach on the benchmark ATIS dataset to investigate, whether using an auxiliary task with class-balanced batch geSFator improves upon a SOTA SLU model. For this purpose, we applied our RoBERTa-based SLU model with vs. without the auxiliary task. Table \ref{tbl:atis_results} presents the results in terms of intent accuracy and F1 for slot filling, which are the standard metrics on ATIS.   
 
%\begin{table}[ht]
%\centering%\small
%\begin{tabular}{l|l|l}
%\hline
%\textbf{Model} & \textbf{Intent acc.} & \textbf{Slot F1}\\
%\hline
%\hline
%Slot-gated \cite{N18-2118}&95.2 &94.1 \\
%Highway LSTM \cite{do19}& 96.8& 95.6\\
%Joint BERT \cite{chen19} &97.5 & 96.0\\
%Joint BERT + CRF \cite{chen19}& 97.9& 96.1\\
%\hline
%Joint RoBERTa + CRF, \emph{RSS}  & 97.4& 95.7\\
%Joint RoBEERTa + CRF, \emph{RSS-CBS} & 97.5 &96.2\\
%\hline
%\end{tabular}
%\caption{Results for CBS on ATIS in comparison to the SOTA.}
%\label{tbl:atis_results}
%\vspace{-0.3cm}
%\end{table}

%Compared to the previously reported SOTA results with a BERT-based model, our baseline model yields higher F1 for slot filling, but lower intent accuracy. As the architectures are similar, this may be mostly due to different optimization and the different BERT models. Applying the auxiliary task improves results of our SOTA baseline model further, both for intent accuracy and slot filling. Thus, data balancing can even improve overall SLU performance in a small-scale set up. Note that the aim of these methods is in particular to boost performance on low-frequency features, which is not necessarily reflected in overall error rates, as the percentage of corresponding samples in the test data is very low.

\section{Results}
%In the following, we first conduct a systematic study regarding data balancing for large-scale SLU on our Alexa feature bootstrapping set up. Subsequently, we explore on the ATIS benchmark datset whether using an auxiliary task with class-balanced batch geSFator can improve upon a SOTA SLU model.
%\subsection{Feature bootstrapping on internal data}

Table \ref{tbl:fb_results} shows the performances of our experimental models on the head intents, and on each of the three low-frequency intents.%, i.e.  \emph{SnoozeNotificationIntent}, \emph{BrowseReminderIntent} and \emph{CancelReminderIntent}. %Note that among the three low-frequency intents, \emph{CancelReminderIntent} is special in that it represents a completely new intent, where no live data are available yet, and hence there are no regular training data for it in our set up.
\begin{table}[t]
%\small
\resizebox{1.05\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Method} & \textbf{Snooze} & \textbf{Browse} & \textbf{Cancel} & \textbf{Head I.}\\
\hline
\hline
\emph{Baseline}  & 22.56 & 64.43 & 55.58 & 4.55\\
\hline
\hline
\emph{Over-sampling} &15.65 & 28.33 & 46.26 & 4.87\\
\emph{Balanced-loss} & 15.24 & 38.42 & 46.26 & 5.07\\
\emph{CBG} & 13.41 & 27.85 & 51.08 & 4.94 \\
\hline
\emph{\textbf{Mul.-CBG} (ours)}  &21.75 & 34.94 & 50.06 & 4.5\\
\hline
\hline
\emph{Data-aug.} & 76.02 & 43.39 & 31.22 & 4.54\\
% CBS 6
\emph{Data-aug.+Over-sampl.} & 15.04 & 40.49 & 30.58 & 4.69 \\
\emph{Data-aug.+Balanced-loss} & 9.55 & 43.18 & 28.11 &   4.73\\
\emph{Data-aug.+CBG} & 7.93 & 40.43 & 30.52 & 5.44\\
\hline
\emph{\textbf{Mul.-CBG+Data-aug.} (ours)} & 15.85 & 42.39 & 54.12 & 4.53\\
%\emph{base},  & mBERT on \emph{base} +  & \multirow{2}{*}{15.85} & \multirow{2}{*}{42.39} & \multirow{2}{*}{54.12} & \multirow{2}{*}{4.53}\\
%\emph{base+MT} & CBS on \emph{base+MT} &&&& \\
\hline
\end{tabular}}
\caption{SemER on three low-frequency intents and on the head intents for data balancing methods on real-world SLU data.}
% SnoozeNotificationIntent, BrowseReminderIntent. and CancelReminderIntent. have 50, 20 and 0 samples in training and validation datasets, respectively.}
\label{tbl:fb_results}
\vspace{-0.9cm}
\end{table}

\subsection{Performance without data augmentation} Performance for all of the low-frequency intents can be improved just by balancing the regular training data. However, for \emph{CBG}, random \emph{over-sampling} and \emph{balanced-loss} methods, the boost in performance comes at the cost of a relative increase in \emph{SemER} for the head intents of at least 7\%. As head intents are much more frequently used by customers, and the customers are used to their comparatively high performance already, such a decrease in performance is usually not acceptable. By contrast, our approach with the class-balanced batch generator boosts performance for all low-frequency features, yielding up to 46\% relative reduction in \emph{SemER} per intent, without over-fitting on the low-frequency classes. Thus, our results suggest that leveraging data balancing techniques in the auxiliary rather than the main task is beneficial. This may be the case, because the model keeps the access to important information about the intent distribution, which is lost when data balancing is applied in the primary task.   
\subsection{Performance with data augmentation} As expected, without using any other techniques, performance is improved when simply adding NMT data (\emph{data-aug.}) to \emph{CancelReminderIntent}, which didn't have any intent samples beforehand. However, for \emph{SnoozeNotificationIntent}, which already had 50 intent samples, simply adding NMT data (\emph{data-aug.}) yields a large increase in \emph{SemER} from 22.5\% to 76.02\%. This highlights the fact that in an evolving system one needs to be careful with maintaining synthetic data. They can be very useful to bootstrap new features when no or few customer feature data are available. However, as they are typically of comparatively low quality, they can decrease performance when they are kept while more and more realistic data become available. While random \emph{over-sampling}, \emph{CBG} and \emph{balanced-loss} can mitigate this problem and improve performance on low-frequency classes, this again comes at the cost of a decrease in performance for the head intents (cf. \emph{data-aug.+over-sampl.}, \emph{data-aug.+CBG} and \emph{data-aug.+balanced-loss}).

\emph{Multi-task-CBG+Data-aug.} indicates performance when NMT data are not added to the primary task training data, but used in the auxiliary task class-balanced batch generator during training only. For \emph{SnoozeNotificationIntent} and \emph{BrowseReminderIntent}, which already have a small number of samples in the realistic training data, performance is improved compared to adding NMT data to the primary task training data without overfitting on the head classes. For \emph{SnoozeNotificationIntent} performance for \emph{Mul.-CBG+Data-aug.} is better than both \emph{Mul.-CBG} without using data augmentation and \emph{data-aug}. This suggests that once a certain amount of realistic intent data becomes available, it's beneficial to leverage NMT data only with \emph{Mul.-CBG+Data-aug}. However, for intents without realistic training data, standard NMT data augmentation is preferable, as the intent cannot be recognized otherwise. Note that this is the case for \emph{CancelReminderIntent} in this experiment. 
\subsection{Does balancing the intent distribution help slot filling?} Interestingly, the intent-based data balancing methods also improve SF performance, as indicated by the results for \emph{CancelReminderIntent} by several methods without including data augmentation, in particular \emph{Mul.-CBG}. Recall that there are no samples for this intent in the regular training data. Hence, the intent cannot be recognized, adding one error to \emph{SemER} for each test utterance evaluation independent of the method (not applying data augmentation). In fact, the improvements for \emph{CancelReminderIntent} are solely resulting from improved SF performance. We attribute this improvement to the fact that slots are shared across several intents and may benefit from intent-based data balancing, as we are using a multi-task model for IC and SF.  

%Overall conclusion is that across all features with CBS we can improve low-freq features while not decreasing (actually increasing) overall performance, and also some MT insights, e.g. that when some live data are available balancing with MT can be more useful than adding MT (which can decrease performance)

%\subsection{Comparison to the state-of-the-art}
%We evaluated our approach on the benchmark ATIS dataset to investigate, whether using an auxiliary task with class-balanced batch geSFator improves upon a SOTA SLU model. For this purpose, we applied our RoBERTa-based SLU model with vs. without the auxiliary task. Table \ref{tbl:atis_results} presents the results in terms of intent accuracy and F1 for slot filling, which are the standard metrics on ATIS.   
 
%\begin{table}[ht]
%\centering%\small
%\begin{tabular}{l|l|l}
%\hline
%\textbf{Model} & \textbf{Intent acc.} & \textbf{Slot F1}\\
%\hline
%\hline
%Slot-gated \cite{N18-2118}&95.2 &94.1 \\
%Highway LSTM \cite{do19}& 96.8& 95.6\\
%Joint BERT \cite{chen19} &97.5 & 96.0\\
%Joint BERT + CRF \cite{chen19}& 97.9& 96.1\\
%\hline
%Joint RoBERTa + CRF, \emph{RSS}  & 97.4& 95.7\\
%Joint RoBEERTa + CRF, \emph{RSS-CBS} & 97.5 &96.2\\
%\hline
%\end{tabular}
%\caption{Results for CBS on ATIS in comparison to the SOTA.}
%\label{tbl:atis_results}
%\vspace{-0.3cm}
%\end{table}

%Compared to the previously reported SOTA results with a BERT-based model, our baseline model yields higher F1 for slot filling, but lower intent accuracy. As the architectures are similar, this may be mostly due to different optimization and the different BERT models. Applying the auxiliary task improves results of our SOTA baseline model further, both for intent accuracy and slot filling. Thus, data balancing can even improve overall SLU performance in a small-scale set up. Note that the aim of these methods is in particular to boost performance on low-frequency features, which is not necessarily reflected in overall error rates, as the percentage of corresponding samples in the test data is very low.
